High-order maximum-entropy collocation methods

This paper considers the approximation of partial differential equations with a point collocation framework based on high-order local maximum-entropy schemes (HOLMES). In this approach, smooth basis functions are computed through an optimization procedure and the strong form of the problem is directly imposed at the collocation points, reducing significantly the computational times with respect to the Galerkin formulation. Furthermore, such a method is truly meshless, since no background integration grids are necessary. The validity of the proposed methodology is verified with supportive numerical examples, where the expected convergence rates are obtained. This includes the approximation of PDEs on domains bounded by implicit and explicit (NURBS) curves, illustrating a direct integration between the geometric modeling and the numerical analysis.

==> table1.tex <==
\begin{tabular}[t]{ |c| c| c| c|  }
\hline
Index $i$ & $x_i$ & $y_i$ & $w_i$\\ \hline
1 & -0.032 & -0.593 & 1.000\\ \hline
2 & 0.070 & -0.545 & 1.028\\ \hline
3 & 0.176 & -0.599 & 1.028\\ \hline
4 & 0.282 & -0.656 & 1.032\\ \hline
5 & 0.388 & -0.717 & 1.035\\ \hline
6 & 0.497 & -0.768 & 1.036\\ \hline
7 & 0.604 & -0.812 & 1.029\\ \hline
8 & 0.684 & -0.776 & 0.970\\ \hline
9 & 0.701 & -0.663 & 0.968\\ \hline
10 & 0.675 & -0.553 & 0.966\\ \hline
11 & 0.634 & -0.448 & 0.966\\ \hline
12 & 0.594 & -0.347 & 0.971\\ \hline
13 & 0.548 & -0.246 & 0.977\\ \hline
14 & 0.569 & -0.145 & 1.005\\ \hline
15 & 0.657 & -0.057 & 1.020\\ \hline
16 & 0.725 & 0.045 & 1.029\\ \hline
17 & 0.793 & 0.149 & 1.038\\ \hline
18 & 0.864 & 0.250 & 1.043\\ \hline
19 & 0.924 & 0.354 & 1.040\\ \hline
20 & 0.916 & 0.438 & 0.974\\ \hline
21 & 0.828 & 0.503 & 0.961\\ \hline
22 & 0.715 & 0.506 & 0.962\\ \hline
23 & 0.607 & 0.509 & 0.965\\ \hline
24 & 0.496 & 0.497 & 0.968\\ \hline
25 & 0.392 & 0.470 & 0.971\\ \hline
26 & 0.286 & 0.469 & 1.003\\ \hline
27 & 0.206 & 0.554 & 1.024\\ \hline
28 & 0.144 & 0.661 & 1.033\\ \hline
29 & 0.078 & 0.765 & 1.040\\ \hline
30 & 0.022 & 0.876 & 1.045\\ \hline
\end{tabular}


==> table2.tex <==
\begin{tabular}[t]{ |c| c| c| c|  }
\hline
Index $i$ & $x_i$ & $y_i$ & $w_i$\\ \hline
31 & -0.049 & 0.976 & 1.044\\ \hline
32 & -0.136 & 0.985 & 0.978\\ \hline
33 & -0.232 & 0.924 & 0.962\\ \hline
34 & -0.251 & 0.816 & 0.968\\ \hline
35 & -0.267 & 0.709 & 0.973\\ \hline
36 & -0.289 & 0.594 & 0.967\\ \hline
37 & -0.297 & 0.482 & 0.966\\ \hline
38 & -0.365 & 0.404 & 1.005\\ \hline
39 & -0.495 & 0.391 & 1.029\\ \hline
40 & -0.615 & 0.378 & 1.033\\ \hline
41 & -0.735 & 0.351 & 1.036\\ \hline
42 & -0.852 & 0.335 & 1.035\\ \hline
43 & -0.963 & 0.308 & 1.023\\ \hline
44 & -0.974 & 0.202 & 0.972\\ \hline
45 & -0.915 & 0.100 & 0.965\\ \hline
46 & -0.824 & 0.037 & 0.966\\ \hline
47 & -0.726 & -0.013 & 0.970\\ \hline
48 & -0.634 & -0.080 & 0.967\\ \hline
49 & -0.532 & -0.130 & 0.967\\ \hline
50 & -0.482 & -0.219 & 0.994\\ \hline
51 & -0.505 & -0.342 & 1.010\\ \hline
52 & -0.532 & -0.458 & 1.013\\ \hline
53 & -0.557 & -0.578 & 1.020\\ \hline
54 & -0.590 & -0.699 & 1.030\\ \hline
55 & -0.604 & -0.821 & 1.030\\ \hline
56 & -0.522 & -0.873 & 0.980\\ \hline
57 & -0.419 & -0.826 & 0.988\\ \hline
58 & -0.320 & -0.774 & 0.991\\ \hline
59 & -0.224 & -0.715 & 0.995\\ \hline
60 & -0.126 & -0.653 & 0.994\\ \hline
\end{tabular}

